Model order reduction in contour integral methods for parametric PDEs

In this paper we discuss a projection model order reduction (MOR) method for a class of parametric linear evolution PDEs, which is based on the application of the Laplace transform. The main advantage of this approach consists in the fact that, differently from time stepping methods, like Runge-Kutta integrators, the Laplace transform allows to compute the solution directly at a given instant, which can be done by approximating the contour integral associated to the inverse Laplace transform by a suitable quadrature formula. In terms of some classical MOR methodology, this determines a significant improvement in the reduction phase - like the one based on the classical proper orthogonal decomposition (POD) - since the number of vectors to which the decomposition applies is drastically reduced as it does not contain all intermediate solutions generated along an integration grid by a time stepping method. We show the effectiveness of the method by some illustrative parabolic PDEs arising from finance and also provide some evidence that the method we propose, when applied to a linear advection equation, does not suffer the problem of slow decay of singular values which instead affects time stepping methods for the numerical approximation of the Cauchy problem arising from space discretization.

==> A Contour Integral Method for MOR/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi
% Packages not SIAM
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{mathrsfs}
\usepackage{algorithm}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{appendix}
\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{color}
\usepackage{bm}
% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% New commands go here
\def\opi{{\mathrm{i}\mkern1mu}}
\def\eps{\epsilon}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\real}{\operatorname*{Re}}
\newcommand{\imag}{\operatorname*{Im}}
\newcommand{\iu}{\mathrm{i}}
\newcommand{\tol}{\mathrm{tol}}
\newcommand{\Id}{\mathrm{I}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bff}{\boldsymbol}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\e}{\mathrm{e}}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\hat}{\widehat}

%%%%%%%
\newcommand\cA{\mathcal{A}}
\newcommand\cD{\mathcal{D}}
\newcommand\cI{\mathcal{I}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}

\newcommand\C{\mathbb{C}}
\newcommand\F{\mathbb{F}}
\newcommand\N{\mathbb{N}}
\newcommand\R{\mathbb{R}}
\newcommand\V{\mathbb{V}}

\newcommand\bA{\bm{A}}
\newcommand\bG{\bm{G}}
\newcommand\bI{\bm{I}}

\newcommand\bb{\bm{b}}
\newcommand\bbf{\bm{f}}
\newcommand\br{\bm{r}}
\newcommand\bu{\bm{u}}

\newcommand\balpha{{\boldsymbol{\alpha}}}
\newcommand\bxi{{\boldsymbol{\xi}}}
\newcommand\bzeta{{\boldsymbol{\zeta}}}

%%%%

\newcommand{\bng}{\color{blue}}
\newcommand{\eng}{\color{black}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
   %% Added by me

% Sets running headers as well as PDF title and authors
\headers%{Contour Integral Methods for time treatment in Certified RBM}
{Model order reduction contour integral methods}{N. Guglielmi, and M. Manucci}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
% \title{Contour Integral Methods for time treatment in Certified Reduced Basis % Methods\thanks{Submitted to the editors 14/01/2022.}}
\title{Model Order Reduction in contour integral methods for parametric PDEs}
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Nicola Guglielmi\thanks{Gran Sasso Science Institute, L'Aquila, IT 
  (\email{nicola.guglielmi@gssi.it}).}
\and Mattia Manucci\thanks{Gran Sasso Science Institute, L'Aquila, IT 
  (\email{mattia.manucci@gssi.it}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

